Enabling Roll-up and Drill-down Operations in News Exploration with Knowledge Graphs for Due Diligence and Risk Management

Efficient news exploration is crucial in real-world applications, particularly within the financial sector, where numerous control and risk assessment tasks rely on the analysis of public news reports. The current processes in this domain predominantly rely on manual efforts, often involving keywordbased searches and the compilation of extensive keyword lists. In this paper, we introduce NCEXPLORER, a framework designed with OLAP-like operations to enhance the news exploration experience. NCEXPLORER empowers users to use roll-up operations for a broader content overview and drill-down operations for detailed insights. These operations are achieved through integration with external knowledge graphs (KGs), encompassing both fact-based and ontology-based structures. This integration significantly augments exploration capabilities, offering a more comprehensive and efficient approach to unveiling the underlying structures and nuances embedded in news content. Extensive empirical studies through master-qualified evaluators on Amazon Mechanical Turk demonstrate NCEXPLORER's superiority over existing state-of-the-art news search methodologies across an array of topic domains, using real-world news datasets.

==> figures/extra_case_studies.tex <==

\begin{adjustbox}{width=1\linewidth}

\begin{tabular}{ |p{1.7cm}|p{1.7cm}|p{3cm}|p{10cm}|} 
    \hline
   Query & Roll-up options & Drill-down options & Results\\
   \hline
   \textcolor{teal}{Asian Countries}, \newline \textcolor{orange}{Stock Market} & \textcolor{orange}{Financial Markets} & Forex Market, \newline  National Oil and Gas Companies & 
   \vspace{-2mm}
   \begin{enumerate}
       \item \textcolor{teal}{Indonesia} Mining \textcolor{orange}{IPO} Vaults Six Shareholders to Billionaire Status 
       \item \textcolor{teal}{China} Tightens Oversight of Program Trading in \textcolor{orange}{Stock Market}
       \item TY Fashion, a Taiwanese-owned garment manufacturer in \textcolor{teal}{Cambodia}, has received approval for listing on the Cambodia \textcolor{orange}{Securities Exchange}
   \end{enumerate}
   \vspace{-3mm}
  \\ \hline
  \textcolor{teal}{Biotechnology Companies of the U.S.}, \newline \textcolor{orange}{M\&A} & \textcolor{orange}{Corporate Finance} & Orphan Drug Companies, \newline Multinational Food Companies &
  \vspace{-2mm}
    \begin{enumerate}
        \item Unilever has expressed interest in acquiring \textcolor{teal}{GlaxoSmithKline}'s consumer healthcare business, a \textcolor{orange}{joint venture} with Pfizer.
        \item  \textcolor{teal}{GSK} leads race to \textcolor{orange}{buy} \textcolor{teal}{Pfizer} unit.
        \item  \textcolor{teal}{Pfizer} to \textcolor{orange}{Purchase} Cancer Drugmaker \textcolor{teal}{Seagen} for \$43 Billion
    \end{enumerate}
    \vspace{-3mm}
  \\ \hline
  \textcolor{teal}{EU countries}, \newline \textcolor{orange}{Labor Disputes} & \textcolor{orange}{social conflicts} & Minimum Wage & 
   \vspace{-2mm}
    \begin{enumerate}
    \item Protesters in \textcolor{teal}{France} demonstrate against President Emmanuel Macron's pension overhaul and the end of the longest transport \textcolor{orange}{strike} in French history.
    \item  \textcolor{teal}{Greece}'s leftist government plans to raise the minimum wage and restore \textcolor{orange}{collective bargaining}, as it seeks to renegotiate the terms of its international bailout
    \item  Amazon faces \textcolor{orange}{strike} of logistical workers in \textcolor{teal}{Germany}
       \end{enumerate}
    \vspace{-3mm}
    \\
 \hline
 \textcolor{teal}{Investment Banks},  \textcolor{orange}{Commercial Crimes} & \textcolor{orange}{Corporate Crimes} & Hedge Funds, \newline  Online Brokerages, \newline Investment Funds, \newline Interest Rates &
 \vspace{-2mm}
    \begin{enumerate}
    \item Broker Faces \textcolor{orange}{Insider Trading} Probe Tied to \textcolor{teal}{Morgan Stanley} Deals.
    \item  Ex-\textcolor{teal}{Morgan Stanley} Adviser Gets Seven Years for Fleecing Clients in \textcolor{orange}{Ponzi Scheme}.
    \item \textcolor{teal}{Deutsche Bank} Said to Probe Senior Russia Employee Over \textcolor{orange}{Bribes}.
    \item \textcolor{teal}{UBS} has lost its appeal against a French \textcolor{orange}{tax evasion} charge.
    \item  \textcolor{teal}{JPMorgan} fined for \textcolor{orange}{wash trades} in oil, gasoline
       \end{enumerate}
    \vspace{-3mm}
    \\ \hline
\end{tabular}
\end{adjustbox}

==> figures/gpt_ndcg_impact.tex <==
\caption{Impact of the GPT mode}
\begin{adjustbox}{width=1\linewidth}

\begin{tabular}{ |c|rrrr|} 
    \hline
  & NDCG@1 & NDCG@5 & NDCG@10 & Overall\\
 \hline
 Lucene & -10.44\% & -2.77\% & -1.40\% & -4.87\% \\
 BERT & 7.18\% & 2.89\% & 1.32\% & 3.80\% \\
 NewsLink & 27.01\% & 6.20\% & 3.08\% & 12.01\% \\
 NewsLink-BERT & 7.05\% & 2.17\% & 1.05\% &3.42\% \\
 NCEXPLORER & 6.75\% & 1.26\% & 0.84\% & 2.95\% \\
 \hline
\end{tabular}
\end{adjustbox}

==> figures/indexing_processor.tex <==

  \begin{tabular}{|p{1.5cm}|p{1cm}|p{5.5cm}|}
    \toprule
    Processor & Output Type & Example \\
    \midrule
    data cleaning & text & Iran Prepares for Elections. Candidates and their supporters on the ground geared up for parliamentary elections in Iran that are slated for Friday. \\
     \hline
    tokenization & word & Iran, prepares, for, elections, candidates, and, their, supporter, on, the ground,... \\
     \hline
    named entity recognition (NER) & (entity) phrase & Iran, prepares, parliamentary elections, candidates, supporter, slate, groud, friday \\
     \hline
    named entity linking (NEL) & linked entity & \textbf{correctly linked entities}: Iran (Q794, Iran), election (Q40231, election), candidates (Q618536, Candidate), supporter(Q725975, Supporter), parliament (Q166747, Parliamentary System) \textbf{incorrectly linked entities}: gear (Q143873, Wheel), slate (Q9394813, Rock) \textbf{unlinked entities}: prepare, ground, friday\\
    \hline
    entity abstraction & KG abstract entities &
    \textbf{Iran} => Iranian Plateau, Azerbaijani-speaking Countries, States and territories established in the 6th century BC, Countries in Asia, G15 national, member state of OPEC, Middle Eastern Countries, Islamic Republics, Country, etc. \textbf{Election} => Election, Politics, etc.
    \textbf{Parliamentary system} => Liberalism, Parliamentary procedure, Political terminology, Types of democracy, etc.\\
%        \hline
%    entity pruning & KG abstract entities &
%    \textbf{Iran} => \xcancel{Iranian Plateau}, \xcancel{Azerbaijani-speaking Countries}, Countries in Asia, G15 national, member state of OPEC, Middle Eastern Countries, Islamic Republics, \xcancel{Country}, etc. \textbf{Election} => Election, \xcancel{Politics}, etc.   \textbf{Parliamentary system} => Liberalism, Parliamentary procedure, %\xcancel{Political terminology}, Types of democracy, etc.\\
    
    
  \bottomrule
\end{tabular}

==> figures/ncgd_human_gpt.tex <==
\begin{center}
\begin{tabular}{ |c|ccc|ccc| } 
    \hline
       & \textbf{Human} & \textbf{GPT-3.5} & \textbf{GPT-4} & \textbf{Human} & \textbf{GPT-3.5} & \textbf{GPT-4}  \\
    \hline
     Topic & \multicolumn{3}{c|}{International Trade} & \multicolumn{3}{c|}{Lawsuits} \\ 

    \hline
    Lucene &  0.571 & 0.333 & 0.397 & 0.608 & 0.136 & 0.382 \\
    BERT &  \underline{0.883} & \textbf{0.950} & 0.823 & \underline{0.853} & \underline{0.666} & \underline{0.764} \\
    NewsLink & 0.641 & 0.167 & 0.424 & 0.422 & 0.072 & 0.189 \\
    NewsLink-BERT & 0.874 & 0.898 & \underline{0.853} & 0.806 & 0.610 & 0.624 \\
    \framework & \textbf{0.951} & \underline{0.903} & \textbf{0.964} & \textbf{0.915} & \textbf{0.881} & \textbf{0.928}  \\
  \hline

  Topic & \multicolumn{3}{c|}{Elections} & \multicolumn{3}{c|}{Mergers \& Acquisitions} \\ 
    \hline
    Lucene &  0.459 & 0.309 & 0.392 & 0.601 & 0.429 & 0.422 \\
    BERT &  0.894 & 0.761 & 0.891 & \textbf{0.835} & 0.686 & 0.538 \\
    NewsLink & 0.465 & 0.330 & 0.254 & 0.469 & 0.006 & 0.126 \\
    NewsLink-BERT & \textbf{0.970} & \textbf{1.000} & \textbf{0.997} & 0.809 & \textbf{0.866} & \underline{0.644} \\
    \framework & \underline{0.965} & \underline{0.911} & \underline{0.969} & \underline{0.824} & \underline{0.700} & \textbf{0.977}  \\

\hline
     Topic & \multicolumn{3}{c|}{International Relations} & \multicolumn{3}{c|}{Labor Dispute} \\ 
    \hline
    Lucene &  0.757 & 0.333 & 0.397 & 0.630 & 0.496 & 0.502 \\
    BERT &  0.917 & 0.950 & 0.823 & 0.441 & 0.509 & 0.153 \\
    NewsLink & 0.760 & 0.167 & 0.424 & 0.489 & 0.186 & 0.357 \\
    NewsLink-BERT & \underline{0.956} & \textbf{0.898} & \underline{0.853} & \underline{0.742} & \underline{0.598} & \underline{0.519} \\
    \framework & \textbf{0.969} & \underline{0.903} & \textbf{0.964} & \textbf{0.979} & \textbf{0.959} & \textbf{0.998}  \\
    \hline
\end{tabular}
\end{center}

==> figures/ndcg_human_gpt_3_column.tex <==
\begin{center}
 \begin{adjustwidth}{-1.5cm}{}
\begin{tabular}{ |c|ccc|ccc|ccc| } 
    \hline
       & \textbf{Human} & \textbf{GPT-3.5} & \textbf{GPT-4} & \textbf{Human} & \textbf{GPT-3.5} & \textbf{GPT-4} & \textbf{Human} & \textbf{GPT-3.5} & \textbf{GPT-4} \\
    \hline
     Topic & \multicolumn{3}{c|}{International Trade} & \multicolumn{3}{c|}{Lawsuits} & \multicolumn{3}{c|}{International Relations}\\ 

    \hline
    Lucene &  0.571 & 0.333 & 0.397 & 0.608 & 0.136 & 0.382 &  0.757 & 0.333 & 0.397\\
    BERT &  \underline{0.883} & \textbf{0.950} & 0.823 & \underline{0.853} & \underline{0.666} & \underline{0.764}  &  0.917 & 0.950 & 0.823 \\
    NewsLink & 0.641 & 0.167 & 0.424 & 0.422 & 0.072 & 0.189 & 0.760 & 0.167 & 0.424\\
    NewsLink-BERT & 0.874 & 0.898 & \underline{0.853} & 0.806 & 0.610 & 0.624 & \underline{0.956} & \textbf{0.898} & \underline{0.853}\\
    \framework & \textbf{0.951} & \underline{0.903} & \textbf{0.964} & \textbf{0.915} & \textbf{0.881} & \textbf{0.928}  & \textbf{0.969} & \underline{0.903} & \textbf{0.964}\\
  \hline

  Topic & \multicolumn{3}{c|}{Elections} & \multicolumn{3}{c|}{Mergers \& Acquisitions} & \multicolumn{3}{c|}{Labor Dispute}\\ 
    \hline
    Lucene &  0.459 & 0.309 & 0.392 & 0.601 & 0.429 & 0.422  & 0.630 & 0.496 & 0.502 \\
    BERT &  0.894 & 0.761 & 0.891 & \textbf{0.835} & 0.686 & 0.538 & 0.441 & 0.509 & 0.153\\
    NewsLink & 0.465 & 0.330 & 0.254 & 0.469 & 0.006 & 0.126 & 0.489 & 0.186 & 0.357\\
    NewsLink-BERT & \textbf{0.970} & \textbf{1.000} & \textbf{0.997} & 0.809 & \textbf{0.866} & \underline{0.644} & \underline{0.742} & \underline{0.598} & \underline{0.519}\\
    \framework & \underline{0.965} & \underline{0.911} & \underline{0.969} & \underline{0.824} & \underline{0.700} & \textbf{0.977}  & \textbf{0.979} & \textbf{0.959} & \textbf{0.998}\\ \hline
\end{tabular}
\end{adjustwidth}
\end{center}

==> figures/ndcg_result_table.tex <==

\begin{tabular}{ |c|ccc|ccc|} 
    \hline
 & NDCG@1 & NDCG@5 & NDCG@10 & NDCG@1 & NDCG@5 & NDCG@10  \\
    \hline
    Topic & \multicolumn{3}{c|}{International Trade} & \multicolumn{3}{c|}{Lawsuits}  \\ 
        \hline
    
    Lucene &  0.705 & 0.571 & 0.745 & 0.578 & 0.608 & 0.772  \\
    BERT &  \underline{0.847} & \underline{0.883} & \underline{0.949} & \textbf{0.837} & \underline{0.853} & \underline{0.936} \\
    NewsLink & 0.807 & 0.641 & 0.792 & 0.341 & 0.422 & 0.645\\
    NewsLink-BERT & 0.812 & 0.874 & 0.945 & 0.641 & 0.806 & 0.887 \\
    \framework & \textbf{0.960} & \textbf{0.951} & \textbf{0.983} & \underline{0.833} & \textbf{0.915} & \textbf{0.957} \\
    \hline


    Topic & \multicolumn{3}{c|}{Elections} & \multicolumn{3}{c|}{Mergers \& Acquisitions} \\ 
  
    \hline
    Lucene &    0.557 & 0.459 & 0.656 & 0.472 & 0.601 & 0.784  \\
    BERT &  0.878 & 0.894 & 0.942 & \textbf{0.754} & \textbf{0.835} & \underline{0.924}\\
    NewsLink & 0.553 & 0.465 & 0.660 & 0.322 & 0.469 & 0.693 \\
    NewsLink-BERT & \textbf{0.941} & \textbf{0.970} & \textbf{0.989} & \underline{0.742} & 0.809 & 0.917  \\
    \framework & \underline{0.918} & \underline{0.956} & \underline{0.977} & 0.690 & \underline{0.824} & \textbf{0.928}  
 \\
    \hline
    Topic & \multicolumn{3}{c|}{International Relations} & \multicolumn{3}{c|}{Labor Dispute} \\ 
    \hline
    Lucene &  \textbf{0.939} & 0.757 & 0.850 & 0.565 & 0.630 & 0.820   \\
    BERT &  0.914 & 0.917 & 0.954 & 0.398 & 0.441 & 0.687 \\
    NewsLink & 0.777 & 0.760 & 0.852 & 0.478 & 0.489 & 0.721  \\
    NewsLink-BERT & 0.893 & \underline{0.956} & \underline{0.977} & \underline{0.720} & \underline{0.742} & \underline{0.897}  \\
    \framework & \underline{0.929} & \underline{0.969} & \textbf{0.984} & \textbf{0.913} & \textbf{0.979} & \textbf{0.987}  
 \\
    \hline
\end{tabular}


==> figures/notations-with-example.tex <==
\begin{tabular}{ |c|p{2.5cm}|p{4cm}| } 
    \toprule
    
    Notation & Description & Example\\
    \midrule
    $\mathcal{G}(\mathcal{V},\mathcal{E}, \mathcal{O})$ & The Knowledge Graph & wikidata, Yago\\ \hline
    $\mathcal{D}(u, v)$ & Distance from node $u$ to node $v$ & $\mathcal{D}$(Boeing, Public Company) = 1\\ \hline
    $P(u \rightarrow v, w)$ & set of paths with length $w$ & $P$(Boeing $\rightarrow$ public company, 1)=\{Boeing $\rightarrow$ public company\} \\ \hline
    $v$ & a node in instance space $\mathcal{V}$ & Boeing \\ \hline
     
    $o$ & a node in concept space $\mathcal{O}$ & countries in Europe\\ \hline
    $\psi(v)$ & concepts mapping function &  $\psi(Boeing)$ = \{public company, wind turbine manufacturers, ...\} \\ \hline
    $\psi\inv(o)$ & instance mapping function & $\psi\inv({Public Company})$ = \{Boeing, Ford motor company, ...\} \\ \hline
    $p$ & pattern, $\{o_1, o_2, ..., o_n\}$, a set of concept entities, it also represents a query & \{conflicts, countries in Europe\}\\
     \hline
    $d$ &  a text document & $d_1$ = Boeing and Ford suspend operations in Russia ...\\
     \hline
     $\Omega$ & concept inverted index $<o, v, d>$ & <Public Company, Boeing, $d_1$> \\ \hline
    $DE({d})$ & document entities set & $DE({doc_1})$ = \{Boeing, Ford motor company, Russia, ...\}\\
     \hline
     $SE({o,d})$ & source entity set.  & $SE({Public Company, doc_1})$=  \{Boeing, Ford motor company\} \\
    \hline
    $SE^{*}({o,d})$ & primary source entity &  $SE^{*}(Public Company,doc_1)= Boeing$ \\
     \hline
    $CE({o,d})$ & context entity set & $CE({Public Company, doc_1})$ = \{Russia, Ukraine, United States, War\} \\ \hline
    $D(p)$ & pattern matching documents & $D$(\{countries in Europe, conflicts\}) = \{d_1, ...\} \\
    
  \bottomrule
\end{tabular}

==> figures/notations.tex <==
\begin{tabular}{ |c|c| } 
    \toprule
    
    Notation & Description\\
    \midrule
    $\mathcal{G}(\mathcal{V},\mathcal{E}, \mathcal{O})$ & The Knowledge Graph\\ \hline
    $\mathcal{D}(u, v)$ & Distance from node $u$ to node $v$ \\ \hline
    $P(u \rightarrow v, w)$ & set of paths with length $w$ \\ \hline
    $v$ & a node in instance space $\mathcal{V}$ \\ \hline
     
    $o$ & a node in concept space $\mathcal{O}$ \\ \hline
    $\psi(v)$ & concepts mapping function  \\ \hline
    $\psi\inv(o)$ & instance mapping function \\ \hline
    $p$ & a concept pattern, $\{o_1, o_2, ..., o_n\}$ \\
     \hline
    $d$ &  a piece of text document \\
     \hline
     $\Omega$ & concept inverted index $<o, v, d>$ \\ \hline
    $DE({d})$ & document entities set \\
     \hline
     $SE({o,d})$ & source entity set \\
    \hline
    $SE^{*}({o,d})$ & primary source entity \\
     \hline
    $CE({o,d})$ & context entity set \\ \hline
    $D(p)$ & pattern matching documents \\
    
  \bottomrule
\end{tabular}

==> figures/productivity_gain_study.tex <==
\caption{
  \framework exploration flow productivity study. This study measures the number of correct answer discovered via two different search tool with the same amount of time.
}
  
 \begin{tabular}{ |P{0.5cm}|P{2.5cm}|P{2cm}|P{1.8cm}| } 
    
    \hline
    
     Task No. & Keyword Search (avg/std) & \framework (avg/std)  & p-value of H1 (n = 10) \\
    \hline
     1 & 0.6/1.07 & 2.7/1.56 & 0.016\\
     2 & 0.5/0.97 & 4.0/1.41 & 0.004\\
     3 & 0.9/0.99 & 2.8/0.46 & 0.001\\
     4 & 0.9/1.10 & 2.7/0.67 & 0.001\\
     5 & 0.7/0.95 & 1.8/0.42 & 0.007 \\
     6 & 1.0/1.56 & 4.5/1.65 & 0.002 \\
     7 & 1.0/1.41 & 4.2/1.03 & 0.001\\
     8 & 1.8/1.03 & 3.3/0.95 & 0.002\\
  
    
  \hline

\end{tabular}

==> figures/relevance_result_table_company.tex <==
\begin{tabular}{ c|ccc|ccc|ccc| ccc } 
    \hline
    Business-related topics & \multicolumn{3}{c|}{Corporate Finance} & \multicolumn{3}{c|}{Lawsuits} &
    \multicolumn{3}{c|}{Law Enforcement} & \multicolumn{3}{c}{Overall} \\ 
        \hline
    Relevance & rel@1 & rel@3 & rel@5 & rel@1 & rel@3 & rel@5 & rel@1 & rel@3 & rel@5 & rel@1 & rel@3 & rel@5\\
    \hline
    Lucene &  0.367 & 0.406 & 0.443 & 0.18 & 0.2 & 0.192 & 0.39 & \underline{0.377} & 0.39 & 0.404 & 0.396 & 0.39 \\
    BERT &  0.517 & 0.461 & 0.442 & 0.12 & 0.113 & 0.116 & \underline{0.59} & 0.313 & 0.282 & \underline{0.516} & 0.353 & 0.343 \\
    NewsLink & 0.367 & 0.394 & 0.453 & \underline{0.28} & \underline{0.293} & 0.248 & 0.25 & 0.337 & \underline{0.46} & 0.332 & 0.387 & 0.452 \\
    NewsLink-BERT &  \underline{0.6} & \underline{0.478} & \underline{0.477} & 0.22 & 0.28 & \underline{0.284} & 0.28 & 0.29 & 0.4 & 0.424 & \underline{0.428} & \underline{0.457} \\
    \framework & \textbf{0.7} & \textbf{0.617} & \textbf{0.617} & \textbf{0.92} & \textbf{0.853} & \textbf{0.892} & \textbf{0.7} & \textbf{0.62} & \textbf{0.616} & \textbf{0.772} & \textbf{0.697} & \textbf{0.70} \\
  \hline
\end{tabular}

==> figures/rollup_example.tex <==


\begin{tabular}{ |p{3cm}| p{12cm}|}
        \hline
        News Article & Lukoil, a \textcolor{orange}{Russian} oil company, calls for an end to the \textcolor{orange}{Ukraine} \textcolor{blue}{war}. \\    \hline

        {Document Entities} & \textcolor{orange}{Russian}, \textcolor{orange}{Ukraine}, \textcolor{blue}{war}\\   \hline

        \textbf{Rollup} {concepts} & \textcolor{orange}{European countries}, \textcolor{blue}{Conflict}\\    \hline

        Implicitly matched documents & 
\vspace{-1mm}
\begin{enumerate}
   \item U.S. weighs \textcolor{orange}{Russian} oil ban as \textcolor{teal}{gas} prices surge and \textcolor{orange}{Ukraine} war grows.
   \item \textcolor{teal}{NATO} accuses \textcolor{orange}{Russia} of using cluster \textcolor{blue}{bombs} in \textcolor{orange}{Ukraine}.
   \item \textcolor{teal}{NATO} rejects intervening in \textcolor{orange}{Ukraine} to avoid the risk of a wider European \textcolor{blue}{war}.
   \item Boeing and Ford halt operations in \textcolor{orange}{Russia} amid escalating \textcolor{orange}{Ukraine} \textcolor{blue}{war}.
   \item What \textcolor{orange}{Putin’s} war could mean for \textcolor{teal}{fossil fuels}.
   \item \textcolor{orange}{France}: Government Introduces \textcolor{blue}{Terrorism} Legislation.
   \item Don't limit \textcolor{orange}{Ukraine} \textcolor{blue}{Refugee} numbers – \textcolor{orange}{Sturgeon}
   \end{enumerate}
   \vspace{-1mm}
        \\ \hline
\end{tabular}


==> figures/subtopic_evaluation_result.tex <==
 \begin{tabular}{ |c|c|c|c| } 

    \hline
    
    Subtopic Rank Components & Company-related Queries & Country-related Queries & Overall\\
    \hline
    C & 2.24 & 2.11 & 2.19\\ \hline
    C + S & 2.03 & 2.23 & 2.11 \\ \hline
    C + S + D & \textbf{1.72} & \textbf{1.64} & \textbf{1.69} \\ 
  \hline

\end{tabular}

==> sections/architecture_backup.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{images/toy-kg.jpg}
    \caption{KG Concept and Instance Spaces}
    \label{fig:kg_toy_sample}
\end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{images/kg-example.pdf}
%     \caption{KG Concept and Instance Spaces}
%     \label{fig:kg_toy_sample}
% \end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{images/architecture-diagram.pdf}
%    \caption{\framework Architecture.}
%    \label{fig:architecture}
%\end{figure}

\framework leverages external KGs for news exploration.
A KG is a multigraph $\mathcal{G}=(\vsetcon \bigcup \vsetins,\esetcon \bigcup \esetins,\onto)$. $\vsetcon$ and $\vsetins$  represent the concept entities and the instance entities respectively, represented by yellow and green nodes in Fig~\ref{fig:kg_toy_sample} respectively. 
Each concept edge in $\esetcon$ links two concept entities, and an instance edge in
$\esetins$ links two instance entities. 
Like~\cite{yang2021newslink}, we add a reversed edge for each original edge so that $\mathcal{G}$ is bidirected.
The associations between the instance space and the concept space are captured by the ontology relation $\onto$. $\onto(c)$ maps a concept entity $c \in \vsetcon$ to a set of instance entities while $\onto^{-1}(v)$ maps an instance entity $v \in \vsetins$ to a set of concept entities.


%The collection of entity nodes are divided into the concept space (i.e., the KG ontology) and the instance space (i.e., the fact network).




\iffalse 
In the following, we introduce the notations  related to the connectivity of the entities in the KG.
\fi

% \noindent\textbf{Connectivity.} Given an instance entity $v$, $N(v)$ denotes the neighbors of $v$ in the instance space. $R_l(v)$ denotes all instance entities that are connected to $v$ by the paths of length $l$. 
% For a concept entity $c$,
% $N(c)$ represents the neighbors of $c$ in the concept space.

% \begin{example}
% Figure~\ref{fig:kg_toy_sample} shows a KG example from wikidata. \kgentity{Boeing}, \kgentity{Biofuel}, and \kgentity{Henry Ford} are instance entities while \kgentity{Public Company} and \kgentity{American Automotive Pioneers} are concept entities. 
% The ontology relation $\onto$ maps \kgentity{Public Company} to two instance entities whereas $\onto^{-1}$ maps \kgentity{Henry Ford} to two concept entities. \kgentity{Public Company} has only one neighbor in the concept space, and \kgentity{Ford Motor Company} has only two neighbors in the instance space. 
% \end{example}


%#95A9D8 #EFCBAF




There are two major components in the architecture of \framework:
semantic \rollup and \drilldown:
% We extract the concepts from each news document in the corpus $\mathcal{D}$ and store the concepts with associated news documents in the forward and inverted index. 
% To explore relevant content of a news article, a user first perform \rollup operations on the news entities to a \emph{concept pattern query} with one or a set of concepts, e.g., roll-up \kgentity{Ukraine} and \kgentity{War} in Figure~\ref{fig:example_query} to a concept pattern that consists of \kgentity{European Countries} and \kgentity{Conflict}.
% With the inverted index, \framework returns news documents that match a concept pattern query and then recommends additional concepts for drill-down explorations. More details of these three components are elaborated below:

% \vspace{1mm}
% \noindent\textbf{News Indexing.}
% Each news document $d\in\mathcal{D}$ is prepossessed by standard NLP techniques.
% We build a linker using the Spacy library~\cite{honnibal2017spacy}. 
% The end product is a set of instance entities extracted from $d$. 
% For each instance entity $v \in d$, 
% we map $v$ to the set of concept entities by the KG ontology relation, i.e., $\onto^{-1}(v)$. Subsequently, we take any concept entity $c \in \onto^{-1}(v)$ and create an inverted index entry $<c,d,cdr(c,d)>$ where $cdr(c,d)$ is the relevance score of concept entity $c$ on document $d$. 
% To ease the presentation, we use entity to denote \emph{instance entity} and concept to denote \emph{concept entity}. 


% Note that the accuracy of entity linking affects the quality of the extracted concepts for a news document. Although improving entity linking accuracy is not the focus of this work, the design of the ranking function $cdr(c,d)$ penalizes irrelevant concepts based on our proposed \emph{ontology relevance} and \emph{context relevance}. The details will be discussed in Sec.~\ref{sec:ranking}.



\vspace{1mm}
\noindent\textbf{Roll-up Operation.}
\framework generates a list of entities from a news document $d$, users then replace one or more entities with KG concepts to form a concept pattern query $Q$. Given such a $Q$, a document $d$ matches $Q$ if for each concept $c \in Q$, there is an entity $v$ in $d$ that $v \in \onto(c)$. In other words, we can find a set of entities in $d$ that match $Q$. 
%In Figure~\ref{fig:example_query}, the 6th result matches the query because \kgentity{France} is associated with \kgentity{Countries in Europe} and \kgentity{Terrorism} is linked to \kgentity{Conflict} by the ontology mapping relation $\onto$. 
The relevance score of a matched document $d$ to $Q$ is the sum of the relevance scores among all concepts in $Q$, i.e.,  
\begin{equation}
	rel(Q,d) = \sum_{c \in Q} cdr(c,d).
\end{equation}
\framework returns all matched documents to the query $Q$, ranked by the relevance scores $rel(Q,\cdot)$. 
%$Q$ is processed by employing efficient list intersections from the inverted index associated with all concepts in $Q$ to retrieve the matched documents.
Furthermore, the entities that match the concepts in $Q$ are annotated to explain why a news document is retrieved. 

\vspace{1mm}
\noindent\textbf{Drill-down Operation.}
Based on the matched news from the \rollup operation,
\framework suggests additional concepts as subtopics to a query $Q$. 
A suggested concept $c'$, as a subtopic of $Q$, enables users to conduct a \emph{drill-down} analysis.
By selecting $c'$, users narrow down the matched news to the augmented query $Q \cup c'$. Since a subtopic must appear as a concept in at least one matched document of $Q$, we can find all candidate subtopics by unionizing the concepts from all matched documents. 
%For efficient query processing, we construct a forward index by storing the concept set of each document, i.e., $<d,c>$. 
%Since there could be a large number of concepts as subtopics, we design an effective ranking scheme and only return top-scored subtopics. 
%The design of the ranking scheme will be discussed in Sec.~\ref{sec:subtopic}.





%\yc{1. How users interact with the system? Using keywords or they can only use a concept pattern to query the system? }

%\yc{2. The output of the system: documents ranked by relevance + subtopic suggestion + outstanding fact (optional).}

%\yc{3. Present the ranking algorithms: (a) ranking documents (assume the concept relevance is known). (b) ranking subtopics: how to find the set of subtopics to suggest?.}

%\yc{We need to discuss why we use AND semantic instead of OR semantic in a bit more detail. I feel that we can emphasize one two points: (1) AND is better for exploration and user studies confirm our approach is better; (2) We can combine a concept pattern with a set of keywords where keyword matches are based on OR semantic. So we are general. }

%Since \framework is designed to be a plugable framework, it uses the same query interface as existing search engines with no special syntax required. The entire concept space can serve as an additional vocabulary set for auto-completion. When a query is sent to \framework, it is transformed into a set of concept entities using the same NLP processors used for indexing except the entity linker performs matching on concept space instead of instance space. The concept entities are joined together using \emph{AND} operator for document retrieval. We choose \emph{AND} over \emph{OR} because of the consistency of search result. For facts retrieval task, a missing keyword will not cause the results to deviate too far from each other. However, this is not the case for exploratory task where the purpose of each additional descriptor is to exclude items from the result. Product search queries on E-commerce sites that do not contain specific brand name are such exploratory tasks. Take the query ``\emph{outfit for children in cold weather}'' as an example. If the concepts in query are joined with \emph{OR}, the search results will contain a wide range of unrelated products such as children books, portable heaters and sports wear. It is cognitively efficient for human brain to analyze a group of related information at a time due to the heavy cost of context switching. For this reason, \emph{AND} is used to maintain the coherency of query result. The behavior of e-commerce sites agrees with this choice.

%From the matching documents of a query, \framework generates a set of subtopics  expanded from instance entities not associated to concepts in the query. These subtopics can serve as filters for the result. They also provide extra, sometimes counter-intuitive, information on the subject. For example, \emph{multinational companies} are not naturally associated with \emph{conflicts between countries} because economic sanction is a very recent concept that has not been included in history book. 


%\begin{table}[h]
%  \caption{Frequent Notations \yc{revise later.}}
%\label{tab:notations}
%\include{figures/notations}
%\end{table}


\begin{comment}
\subsection{Domain oriented document retrieval}
To map a document to multiple related domains, we first pre-process text documents with a series of natural language processing (NLP) tools like tokenization, parts-of-speech tagging, stemming, named entity recognition (NER) and named entity linking (NEL). We use open-source libraries for most of the tools except for NEL. Our internal NEL implementation links document phrases to DBPedia nodes using a self-trained neural network model and DBPedia Spotlight\cite{mendes2011dbpedialinking}. The quality of NEL greatly impact the system performance, however, it is not the focus of the work. We address the issue of NEL errors in domain relevance ranking step which will be described later.

NEL transforms a text document to entities in the KG instance space while the topical domains resides in KG concept space. The KG expansion processor extends instance entities to concept entities via graph traversals along selected edge types. These edge types are KG dependent. In DBPedia, the edge types are \textit{type, subject, boarder and hypernym}. Graph traversal algorithms like breadth-first search, depth-first search, random walk with restart\cite{tong2006fast}, etc, can all be used here depends on KG characteristics and computational budget. The set of concept entities visited during expansion are added to the inverted index as relevant domains for a document.

The domain based inverted index is similar to the term based index except when there are more than one topic in the query, such as \textit{elections in African countries}. Keyword matching systems use \textbf{OR} to join multiple terms whereas DORE uses \textbf{AND} to combine topics. This is based on the assumption that when a user user involves more concepts into a query, the intent is to narrow down the result instead of broaden it.
\end{comment}


==> sections/backup.tex <==

The major components are: the Natural Language Processing (NLP), the Entity Abstraction (EA) component and News Abstraction Search (NEA) component. For NLP component, this research does not propose any novel idea but it is crucial to generate high quality input data for our abstraction algorithm. We will still describe the details for reproducibility purpose. EA and NEA are the main contributions of this work.

\subsection{The NLP stage}
The responsibility of NLP task is to extract entities like person, organization, location from a text document and link the surface form to a node in the KG.
To achieve this task, we follows the standard text processing pipeline of tokenisation, named entity recognition and named entity linking. For named entity linking, we trained a vector based model with the spaCy library\cite{honnibal2017spacy} and combine with the result from DBPedia Spotlight\cite{mendes2011dbpedia}. For each news article, we concatenate the title with first two sentences to feed into the NLP component. The purpose is to balance data processing time and capturing enough important entities. We think it is reasonable to assume most important entities will appear in first two sentences of a news article. Due to the incompleteness of KG, not all named entities can be linked to a node in KG. Unlinked entities are left out from abstraction step and pass straight to search step. For example in Figure ~\ref{fig:sample-ner-nel}, eight unique entities are extracted from the document. Among eight recognized entities, seven of them are able to be mapped to an entry in KG. Figure ~\ref{fig:sample-kg-entity} shows an entry in DBPedia identified from news article in Figure ~\ref{fig:abstraction-serach-query}.


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/sample-ner-nel.png}
  \caption{Result of NLP Stage. Eight unique entities are recognized and seven are linked to KG.}
  \label{fig:sample-ner-nel}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/sample-kg-entity2.png}
  \caption{A sample linked entity in DBPedia.}
  \label{fig:sample-kg-entity}
\end{figure}

\subsection{The EA stage} \label{sec:ea-stage}
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/abstraction-candidates.png}
  \caption{Abstraction candidates for entity \textit{Amazon (company)}}
  \label{fig:abstraction-candidates-amazon}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/software-companies-in-seattle.png}
  \caption{KG nodes linked to \textit{software companies based in Seattle}}
  \label{fig:software-company-based-in-seattle}
\end{figure}



\begin{table*}[t]
  \caption{Sample entity abstractions and their robustness \& semantic closeness score}
  \label{tab:entity-abstractions-robustness-sc}
  \begin{tabular}{ccc}
    \toprule
    Entity Abstraction&Semantic Closeness & Robustness Score \\
    \midrule
    Biopharmaceutical companies & 0.23 & 206 \\
    2103 Initial Public Offerings & 0.19 & 31 \\
    Orphan Drug Companies & 0.19 & 513 \\
    Corporate spin-offs & 0.17 & 307 \\
  \bottomrule
\end{tabular}
\end{table*}
The EA component expands each entity to a set of abstraction candidates. We uses DBPedia data for this step. Given a linked entity, all neighbours with edge type \textit{rdf:type} and \textit{dct:subject} are selected as abstraction candidates which corresponds to ‘categories’ in Wikipedia. For some entities, the number of abstraction candidates can be large. Each abstraction has different levels of generalness. For example, Figure ~\ref{fig:abstraction-candidates-amazon} shows the list of abstraction candidates for Amazon Inc. \textit{Thing, company, organization} represent highly general idea. These nodes have high degree in KG and similarity between their connected entities are low. On the other end of the spectrum, as shown in Figure ~\ref{fig:software-company-based-in-seattle}, the abstraction \textit{software companies based in Seattle} only has 25 neighbors. It scores low on generalness and similarity between its linked nodes are high. A more general abstraction fetches bigger number of query results but there are less semantic similarities between the results. A closer semantic relationship will decrease the diversity of matching documents. We want to find a balance between robustness and the semantic closeness of query results because neither end of the spectrum are meaningful for the news search task. Robustness can be calculated by directly counting number of documents an abstraction is related to. For semantic closeness score (SC), we use the average JaccardIndex between linked entities as an approximation. As shown in Equation ~\ref{abstraction_semantic_closeness_score}, \textit{N} is the set of entities linked to abstraction \textit{A}. For each pair of entities in \textit{N}, we calculate the JaccardIndex to measure their closeness. The average JaccardIndex among all the neighbors are used to represent Semantic Closeness. For abstraction node with high degrees (more than 100), we randomly sample 100 neighbors to reduce computation complexity. The mathematical product of SC and robustness score provides a balanced view on the quality of an abstraction. Only top K abstractions will be retained for downstream task. K is a hyper-parameter customizable by the system user. This is a one time meta data calculating task. The computation cost will be amortized over future updates as new documents will only update parameters on a small set of entities. 

Table ~\ref{tab:entity-abstractions-robustness-sc} shows a few sample abstractions. \textit{Biopharmaceutical companies} has both high semantic closeness score and robustness scores. In contrast, \textit{2013 Initial Public Offerings} scores lower on both metric. Thus, it will not be prioritized by the system as an abstraction candidate.
\begin{equation}\label{abstraction_semantic_closeness_score}
    SC(A)=\frac{1}{\vert N\vert}\sum_{m,n \in N, m \neq n}JaccardIndex(m,n)
\end{equation}

JaccardIndex is our first attempt of similarity measurements due to its simplicity. However it might not be the optimal choice because it only considers KG information and ignores other entities extracted from the same document. For example, considering the news "Jeff Bezos to step down as Amazon's CEO" with \textit{Jeff Bezos} and \textit{Amazon} as linked entities. If we only use JaccardIndex, the abstraction of entity \textit{Jeff Bezos} is likely to be one of \textit{Billionaire}, \textit{Business Man}, \textit{Amazon.com People}. However, preference should be given to \textit{American Technology Chief Executives} or \textit{American Technology Company Founders} because this is how it links to the other entity \textit{Amazon.com}.


\begin{table}
  \caption{Evaluation of abstraction of entity \textit{Jeff Bezos} in the context of \textit{Amazon} entity}
  \label{tab:entity-abstractions-evaluation}
  \begin{tabular}{p{4cm}p{2cm}p{2cm}}
    \toprule
    Abstraction & Inter-document relatedness & Semantic Closeness Score\\
    \midrule
    Billionaire & Low & High \\
    American Technology Chief Executives & High & High \\
    People in Space Industry & Low & Low \\
  \bottomrule
\end{tabular}
\end{table}


\subsection{The NS stage}

\begin{table*}[t]
  \caption{For each news article, we obtain a table of entities and their abstractions}
  \label{tab:possible-news-abstractions}
  \begin{tabular}{lllll}
    \toprule
    Entity & AbbVie & JAK1 & Rheumatoid Arthritis & ...\\
    \midrule
    Abstraction & Biopharmaceutical Companies & BioChemEntity & Medical Condition & ... \\
    Abstraction & S\&P 100 & Protein & Thing & ...\\
    Abstraction & Company & Thing & Category:Arthritis & ... \\
    Abstraction & ... & ... & ... & ... \\
  \bottomrule
\end{tabular}
\end{table*}

After EA stage, we obtain a set of entities and their corresponding abstractions for each news document. Table ~\ref{tab:possible-news-abstractions} shows an example. The number of recognized entities for each news are different from the other news. The set size of each entity is also not fixed. These abstractions are used to build the index for document search application. As shown in screenshot ~\ref{fig:abstraction-serach-query}, each recognized entities has a list of abstractions for users to chose. Query results are documents containing entities with abstractions equal or is a subset of the chosen abstraction set. The matched abstraction set are appended to each result so that users know exactly how the results are generated. Currently, among all possible abstractions, the system randomly selects one and uses that as query input. For an abstraction, the system first fetches entities linked to the abstraction. It then uses those entities to query document. This two step process is not as efficient as token based inverted index search in common search engines. It is due to the fact that text-document mapping is one-to-one but abstraction-document mapping is many-to-one. For example, in Table ~\ref{tab:possible-news-abstractions}, if we construct a direct abstraction-document mapping, there will be an entry of <Biopharmaceutical Companies, document\_id\_1> as well as <S\&P 100, document\_id\_1>, <Company, document\_id\_1>. All the three entries are linked to the same entity \textit{AbbVie}. If these entries are used as inverted index, query results will following different scenarios: 1. a news document with four matched abstractions because AbbVie appears in the text. 2. a news document with four matched abstractions from two different companies, one smaller Biopharmaceutical company and another S\&P 100 company like Apple Inc. 3. a news document with four matched abstractions from four different entities. Although all of the cases are related to the original document in some way. The closeness are very different. In current design, we only consider case 3. In future, we aim to include all of them in the results but score them differently.




\subsection{Frequent Itemset Mining}
After each news document is transformed in to a set of abstractions, we can then start mining frequently occurring patterns, associations or correlations from this dataset. Association rule mining is a procedure commonly used to mine patterns in transactional databases. The classic anecdote is in supermarket dataset where beer and diaper frequently appear in a common receipt. In order to define importance, two parameters are supplied as input to the procedure to constrain rule significance: support and confidence. Let \textit{X}, \textit{Y} be itemsets and \textit{T} represents transactional dataset. \(X \Rightarrow Y\) is an association rule. Support indicates how frequently the pattern appears in the dataset, i.e. the fraction of transactions in \textit{T} which contains the itemset \textit{X}. Confidence shows how often the rule has been found to be true, i.e. the confidence of \(X \Rightarrow Y\) is the portion of transactions in \textit{T} that contains \textit{X} also contains \textit{Y}. Many algorithms haven been proposed to generate association rules. Apriori \cite{agrawal1994fast} is the most well-known work in this area, it uses a BFS approach to count the support of itemset and exploit the downward closure property to prune candidates. FP-growth \cite{han2000mining} is an improved version of the Apriori, created to reduce the amount of disk I/O caused by multiple database scans when checking support constrains. 

In our work, the news abstractions cannot be feed directly to association rule algorithms due to the one-to-many document-abstraction mapping explained earlier. If we simply concatenate all abstractions from each document, there is a chance a frequent pattern is generated from a small number of documents but each document has a large number of abstractions. In order to generate meaningful results, a single abstraction needs to be selected from each document. Making the selection is not an easy task. It requires knowledge from both local and global information. Local information helps select an abstraction by considering the relationship between different entities in the same document. Global information takes into consideration the entity distribution across different documents and help coordinating abstraction selection in a centralized manner to boost support. It is critical to find the right weight for local and global force when performing abstraction selection. If local information weights too much, the result will be fragmented with many low support itemsets. On the other hand, if global information over rules, the result will be many meaningless high support association rules such as \textit{<Organization, Thing, Person>}. These highly abstracted frequent itemsets neither help journalists to discover interesting stories to report nor enhance readers' information consuming experience.

In preliminary exploratory work, we applied Apriori \cite{agrawal1994fast} algorithm to randomly selected news abstractions. The list below showed an example frequent pattern \textbf{<Currency, Monetary Policy, National and Language>} and a few associated documents.

\begin{itemize}
  \item \textbf{Euro} struggles ahead of \textbf{ECB policy meeting} on Thursday.
  \item \textbf{Ringgit} hits 6-year low; central bank of \textbf{Indonesia} to keep \textbf{interest rates}.
  \item Copper prices slipped on Tuesday as excitement over a weekend \textbf{interest rate} cut in top consumer \textbf{China} dissipated, and as the \textbf{dollar} was seen gaining strength.
\end{itemize}

Intuitively, we can understand the abstraction is about governments and monetary policy. This can be useful in several ways. First, this can be an automated method for tagging a document. The readers can subscribe to a combination of the abstraction tags and start receiving notifications on new documents with all matching abstractions. Compare to existing manual based document tagging, it is more objective and efficient. It can also retrospectively tag historical documents in an efficient manner. Second, most documents are associated with a temporal meta data like timestamp. This time information can transform document counts of a frequent pattern into a time series data which can be further combined with other time series index for correlation analysis. For instance, if we plot the frequency of \textbf{<Currency, Monetary Policy, National and Language>} together with global macro economic matrices like international trade volume, commodity prices, we should be able to discover some correlations.

\section{Evaluation}
As this is a work-in-progress report, we are not able to show all experiment results yet. Here we will describe the set of experiments.

\subsection{Dataset}
1) news dataset: We conduct our experiment two news datasets: Reuters and seekingalpha.com. Reuters cover a wide range of topics while seekingalpha.com most focuses on finantial news reporting. We feed the title and first two sentences of each news article for NER and NEL process. We filter out all documents we cannot find at least one linked KG entity.

2) Knowledge Graph: we use DBPedia\cite{mendes2011dbpedia} to perform abstraction task.

3) Benchmarks: we will evaluate our implementation against these alternatives:

\begin{itemize}
  \item \textbf{AbstractionSearch}: our proposed method to retrive similar documents via similar entity abstractions.
  \item \textbf{Doc2Vec\cite{le2014distributed}}: A neuro network model that transform a text document into a dense vector representation. We will use an opensource implementation Gensim \footnote{https://radimrehurek.com/gensim/models/doc2vec.html} to train a model with 500 dimensions.
  \item \textbf{Sentence-BERT (SBERT)\cite{reimers-2019-sentence-bert}}: A modification of the state-of-the-art BERT model. It uses siamese and triplet network structures to produce sentence embeddings. We uses the framework\footnote{https://www.sbert.net/} published by the original research team.
  \item \textbf{ElasticSearch}: an opensource full-text search engine built on top of Apache Lucene\cite{mccandless2010lucene}. We use the default Okapi BM25\cite{robertson2009probabilistic} as similarity ranking function.
\end{itemize}

4) Platform and Implementation
The NLP component is implemented in Python 3.7 with spaCy library. We trained our own NEL model from Wikidata. News search and association rule mining is also implemented in python 3.7.

\subsection{Evaluation Task}
We simulate real world short phrase search scenario by using a news title as query Q and uses that to retrieve results \(\{R_1, R_2, ..., R_k\}\) which are similar to Q.

\section{Future Work}
As next step of this work, there are two tasks we plan to explore more on. First, among all possible abstractions combinations for a news article, we aim to recommend one most interesting abstractions set as the default query to generate similar documents. We plan to conduct experiments with existing similarity algorithms to demonstrate our approach increases result robustness without compromising semantic relatedness. Second, we aim to mine meaningful patterns from the collection of abstraction sets. For example, Figure ~\ref{fig:sample-abstraction-patterns} shows two sample patterns. It is not difficult to understand the abstractions set <\textit{Medical Condition}, \textit{Clinical Research Assets}, \textit{Corporate spin-offs}, \textit{Medical terminology}> is about medical drug development and the abstractions set <\textit{rating}, \textit{raise}, \textit{Pricing}, \textit{maintain}> is about financial organization announcements. These patterns are useful in several ways such as helping people visualize the major events given a period of time and how certain events gain or lose momentum over time. If paired with other time series data like economic index, journalists are able to identify some correlations that are difficult to identify otherwise. One of the example we discovered from previous exploratory work is \textit{mergers and acquisitions} correlates with stock market volatility of affected companies.




\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/sample-abstractions.png}
  \caption{KG nodes linked to \textit{Sample abstraction patterns}}
  \label{fig:sample-abstraction-patterns}
\end{figure}

==> sections/problem_definition.tex <==

\begin{table}
  \caption{Sample KG edges and nodes }
  \label{tab:abstract-concrete-kg-node}
  \include{figures/sample_kg_entities}
\end{table}

In this paper, we use \(\mathcal{D}\) to denote the set of corpus. KG can be considered as a set of RDF\footnote{https://www.w3.org/TR/rdf-primer/} triples in the form of <subject, predicate, object>. In graph structure, subject and object are nodes and predicate represent edges. A KG node can either be a concrete term of person, organization, location or an event type, an object category, a parent-child class in an ontology. KG nodes type can be differentiated by the edge pointing to them as shown in Table ~\ref{tab:abstract-concrete-kg-node}. 

For each individual document d, the set of linked entities are denoted as \(E = \{e_1, e_2, ... e_n\}\). As shown in Figure ~\ref{fig:document_entities_abstractions}, each entity has an abstraction set represented as \(Abstraction({e}) = \{a_{e_1}, a_{e_2}, ..., a_{e_k}\}\).

Note there might be overlapping of abstractions for different entities. For example, Amazon Inc. and Google Inc. can appear in the same piece of news and they share common abstractions: Cloud computing providers, Multinational companies headquartered in the United States and Mobile phone manufacturers.

Last, we define a pattern \(\mathcal{p}\) as the set of one or more distinct abstractions, e.g. {Elections, Countries in Asia}, {Lawsuits, Software companies in the United States}.

Our goal of the research include: 

\begin{itemize}
    \item given a set of abstract topics as query, find all related documents sorted by relevance level.
    \item suggest meaningful sub-patterns for each query to help users navigating the domain of their analytical tasks.
    \item for each pattern, automatically discover interesting (outstanding) attributes among related entities. These outstanding facts can serve as entertainments for general users or data sources for professionals like journalist to craft stories from a fresh angle.
\end{itemize}


\begin{figure}
\include{figures/document_entitiy_abstractions}
\caption{Document Entities and Abstractions}
\label{fig:document_entities_abstractions}
\end{figure}

==> sections/ranking_backup.tex <==
%\def\fullversion{0}

% In this section, we first discuss the ranking schemes in \framework: Section~\ref{sec:ranking} presents the relevance score between a concept $c$ and a document $d$, i.e., $cdr(c,d)$; Section~\ref{sec:subtopic} presents the subtopic score for a concept $c$ and a query $Q$, i.e., $sbr(c,Q)$. In Section~\ref{sec:sample} we discuss how to efficiently compute the scores with sampling techniques.
%Before moving on, all frequent notations are summarized in Table~\ref{tab:notations}.

% removed from v1
% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=\linewidth]{images/abstraction_document_relevance_score_simple.pdf}
% 	\vspace{-2em}
% 	\caption{\framework context relevance score computation.}
% 	\vspace{-1em}
% 	\label{fig:notations_example}
% \end{figure*}




\subsection{Connectivity Score Estimation}
The connectivity score can be computationally expensive due to the massive number of path enumerations for each pair of entities and existing studies on s-t path enumeration can only produce \emph{polynomial delay} algorithms~\cite{qin2019towards,sun2021pathenum}. Inspired by the sampling approaches for online join aggregation queries~\cite{li2016wander,zhao2018random,park2020g}, we devise 
a single random walk estimator. 
To start a random walk, we first sample a source entity $u$ from all entities that map to the concept $c$, and a target entity $v$ from the corresponding context entities.
A \emph{non-repeating} random walk $r(u,v)$ from $u$ tries to reach $v$ samples via at most $\tau$ distinct nodes. 
Let $u_i$ denote the $i$th node sampled by a random walk starting from the source $u$ and $N(u_i)$ is the number of eligible neighbors of $u_i$ to be sampled, we define the following sample estimator:
\begin{equation}
	r(u,v) = \mathcal{I}(u,v) \cdot |\onto(c)| \cdot \beta^{l-1} \cdot \displaystyle \prod_{i=1}^{l-1} N(u_i)
\end{equation}
where $\mathcal{I}(u,v)$ is an indicator random walk: it returns $1$ if $u$ reaches $v$ at the $l$-th sampled node for any $l \leq \tau$; otherwise, it returns $0$. 

The sampling process may suffer from slow convergence, especially when many of the sampled paths cannot reach the target context entity $v$.  
To enable faster convergence, we build a reachability index~\cite{cheng2014efficient} on the KG instance space and only sample eligible neighbors that satisfy the hop constraint. 
%We run multiple random walks and use the sample mean to approximate the connectivity score, i.e., $\widehat{conn}(c,d) = \frac{1}{\theta}\sum_{j=1}^\theta r_j$. 
The following theorem ensures our sample approach is unbiased.
\begin{theorem}
	$r(\cdot,\cdot)$ is an unbiased estimator to $conn(c,d)$, i.e., $\mathbb{E}[r(\cdot,\cdot)] = conn(c,d)$ where the randomness is taken over the source $u$ and target $v$ as well as the random walk from $u$ to $v$. 
\end{theorem}
Proof Sketch. $conn(c,d)$ is a weighted sum of all the paths connecting an entity node $u \in \onto(c)$ and a context entity $v \in CE(c,d)$ subject to a hop constraint of $\tau$. For each path $s=\{u_1=u,u_2,u_3,...,u_l=v\}$ that connects $u$ and $v$, the probability of $s$  being sampled is $\mathbb{P}(s)=(|\onto(c)|\cdot|CE(c,d)|\cdot\prod_{i}^{l-1} N(s_i))^{-1}$.
Thus, we can use the Horvitz–Thompson estimator~\cite{HTestimator} to approximate the population sum without bias. 


\subsection{Drill-down Exploration Rank}\label{sec:subtopic}
%A large number of relevant documents can be retrieved for a concept pattern query $Q$ with the roll-up operation. 
%To facilitate users in navigating the results with a concept-centric approach, \framework automatically detects related concepts in the retrieved documents as the suggested subtopics for users to perform \emph{drill-down} analysis. 

\framework can retrieve a significant amount of relevant documents for a concept query $Q$ using the roll-up operation. To aid users in navigating the results, \framework identifies related concepts in the retrieved documents and suggests them as subtopics for users to conduct \emph{drill-down} analysis. Let $\mathcal{D}(Q)$ denote the set of retrieved documents for $Q$ and a candidate subtopic is a concept $c$ such that there is an instance entity $v \in \onto(c)$ appearing in one of the documents $d \in \mathcal{D}(Q)$.
%For example, \kgentity{Multinational Companies with HQ in the U.S} is a candidate subtopic for the query in Figure~\ref{fig:example_query} since \kgentity{Boeing} and \kgentity{Ford Motor Company} are matches of the subtopic, and they appear in the news retrieved for the query. 
We develop a score $sbr(\cdot,Q)$ over candidate subtopics and only suggest top-scored subtopics for $Q$. 
There are three key perspectives considered in $sbr(\cdot,Q)$ as below:
\begin{equation}
	sbr(c,Q)=coverage(c,Q) \cdot specificity(c) \cdot diversity(c,Q)
\end{equation}

\begin{itemize}[leftmargin=5mm]


	%\item \textbf{Coverage.} Among all the documents retrieved for $Q$, a niche subtopic that is only related to a small number is less attractive to users for exploration. Thus, we use the total relevance of a concept to all the documents in $\mathcal{D}(Q)$ as the coverage score, i.e., $coverage(c,Q)=\sum_{d \in \mathcal{D}(Q)} cdr(c,d)$. 
    \item \textbf{Coverage.} 
    %To help users explore the retrieved documents for a concept pattern query Q, it is important to suggest subtopics that are relevant to a significant number of documents. 
    The coverage score of a subtopic $c$ is calculated as the sum of the relevance scores $cdr(c, d)$ for all documents $d$ in $\mathcal{D}(Q)$. This ensures that only subtopics that are highly relevant to a large number of documents are suggested to the user for further exploration: $coverage(c,Q)=\sum_{d \in \mathcal{D}(Q)} cdr(c,d)$.
	%\item \textbf{Specificity.} Similar to the ontology relevance, a broad concept that matches a large number of entities is less desirable as it could lead to suggesting a trivial subtopic, such as \kgentity{Person}. Hence, we use $specificity(c)=\log(|\vsetins|/|\onto(c)|)$ to prioritize concepts with higher specificity scores. 
 \item \textbf{Specificity.} To avoid suggesting trivial subtopics like \kgentity{Person} which may match a large number of entities, we prioritize concepts with higher specificity scores using the formula $specificity(c)=\log(|\vsetins|/|\onto(c)|)$. 
%similar to how we prioritize based on ontology relevance.
	

 \item \textbf{Diversity.} The diversity score calculates the average number of distinct entities mapped to the concept $c$ among all the documents relevant to $Q \cup \{c\}$: $diversity(c,Q) = \frac{|\bigcup_{d \in \mathcal{D}(Q)} ME(c,d)|
		}{|\mathcal{D}(Q \cup \{c\})|}$.
 % \begin{equation}
	% 	diversity(c,Q) = \frac{|\bigcup_{d \in \mathcal{D}(Q)} ME(c,d)|
	% 	}{|\mathcal{D}(Q \cup \{c\})|}
	% \end{equation} 
 %We normalize the score as the average number of distinct entities mapped to the concept $c$ among all the documents relevant to $Q \cup \{c\}$. 
 This helps ensure fairness in the suggested concepts and prevents results from being biased toward concepts that match a small set of popular entities.
\end{itemize}


\if\fullversion1
\subsection{Connectivity Score Estimation}\label{sec:sample}
Although the connectivity score can effectively detect relevant concepts for both news matching and news exploration purposes, the score is prohibitively expensive to compute for two reasons. 
First, consider the rightmost summation of Equation~\ref{eq:conn}, it requires to enumerate all simple paths up to $\tau$-hop that connect a context entity with any KG instance entity mapped to concept $c$. The path enumeration of each entity pair is expensive as existing studies on s-t path enumeration can only produce \emph{polynomial delay} algorithms such that the time between finding two successive path results is bounded by a polynomial function
of the input size in the worst case~\cite{qin2019towards,sun2021pathenum}.
Second, there is a massive number of s-t path enumeration tasks to execute for just processing one news document in the indexing component of \framework.
For each ontology-relevant concept $c$, we need to compute the context relevance score between $c$ and each context entity in $d$ for creating the index entry $<c,d,cdr(c,d)>$. Furthermore, the number of instance entities that map to $c$ in the KG is massive, especially for broad concepts like \kgentity{Company} and \kgentity{People}. 


Inspired by the sampling approaches for online join aggregation queries~\cite{li2016wander,zhao2018random,park2020g}, we devise 
a single random walk estimator to reduce the expensive cost of computing the context relevance scores.  
To start a random walk, we first sample a source entity $u$ from all entities that map to the concept $c$, and a target entity $v$ from the corresponding context entities.
A \emph{non-repeating} random walk $r(u,v)$ from $u$ tries to reach $v$ samples via at most $\tau$ distinct nodes. 
Let $u_i$ denote the $i$th node sampled by a random walk starting from the source $u$ and $N(u_i)$ is the number of eligible neighbors of $u_i$ to be sampled, we define the following sample estimator:
\begin{equation}
	r(u,v) = \mathcal{I}(u,v) \cdot |\onto(c)| \cdot \beta^{l-1} \cdot \displaystyle \prod_{i=1}^{l-1} N(u_i)
\end{equation}
where $\mathcal{I}(u,v)$ is an indicator random walk: it returns $1$ if $u$ reaches $v$ at the $l$-th sampled node for any $l \leq \tau$; otherwise, it returns $0$.

We run multiple random walks and use the sample mean to approximate the connectivity score, i.e., $\widehat{conn}(c,d) = \frac{1}{\theta}\sum_{j=1}^\theta r_j$. 


The following theorem ensures our sample approach is unbiased.
\begin{theorem}
\label{unbiased_estimator}
	$r(\cdot,\cdot)$ is an unbiased estimator to $conn(c,d)$, i.e., $\mathbb{E}[r(\cdot,\cdot)] = conn(c,d)$ where the randomness is taken over the source $u$ and target $v$ as well as the random walk from $u$ to $v$. 
 
\end{theorem}

\noindent
Proof Sketch. $conn(c,d)$ is a weighted sum of all the paths connecting an entity node $u \in \onto(c)$ and a context entity $v \in CE(c,d)$ subject to a hop constraint of $\tau$. For each path $s=\{u_1=u,u_2,u_3,...,u_l=v\}$ that connects $u$ and $v$, the probability of $s$  being sampled is $\mathbb{P}(s)=(|\onto(c)|\cdot|CE(c,d)|\cdot\prod_{i}^{l-1} N(s_i))^{-1}$.
Thus, we can use the Horvitz–Thompson estimator~\cite{HTestimator} to approximate the population sum without bias. 


\begin{algorithm2e}[t]
   % \LinesNumbered
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{KG $\mathcal{G}$, concept $c$, document $d$, sample size $\theta$}
	\Output{the estimated connectivity $est$}
        $est \gets 0$; \\
	\While{there are less than $\theta$ random walks}{
		  $l \gets 1$; $p \gets 1.0$; \\
		  $u_l \gets$ a random entity in $\onto(c)$; \\
		  $v \gets$ a random entity in $CE(c,d)$; \\
		  \While{$l \leq \tau$}{
			$count \gets 0$; \\ 
			\ForEach{$n \in N(u_l)$}{
				\If{$hop(n,v) \leq \tau-l$ \label{alg:hop-constrain}}{
					$count \gets count + 1$; \\
					$u_{l+1} \gets n$ with probability $\frac{1}{count}$;\label{alg:single-scan}
				}				
			}
			$p \gets \frac{p}{count}$; \\
			$l \gets l+1$; \\
			\textbf{break} on $u_{l} = v$; 
		}
		\If{$u_{l} = v$}{
			$est \gets est + \frac{\beta^{l-1}}{p}$;
		}
	}
	\Return {$\frac{est \cdot |\onto(c)|}{\theta} $.} \\
	\caption{Random walk estimator with k-hop index.} 
	\label{algo:samplekhop}
\end{algorithm2e}


\vspace{1mm}
\noindent\textbf{Convergence Optimization}.~Although we devise an unbiased estimator for the connectivity score, the sampling process may suffer from slow convergence, especially when many of the sampled paths cannot reach the target context entity $v$.  
To enable faster convergence, we build a reachability index~\cite{cheng2014efficient} on the KG instance space and only sample eligible neighbors that satisfy the hop constraint. We present our sampling approach with the k-hop reachability index in Algorithm~\ref{algo:samplekhop}.
For each random walk, we first sample the source $u_1$ and the target $v$. 
Subsequently, we iteratively sample the next node $u_{l+1}$ by scanning the neighbors of $u_l$. With the help of the k-hop index, we first check if a neighbor $n$ can reach $v$ within the hop constraint of $\tau-l$ (Line \ref{alg:hop-constrain})
Then, we uniformly sample eligible neighbors by a Reservoir sampler, which only requires a single scan of the neighbors (Line \ref{alg:single-scan})
A random walk terminates when either the target $v$ is sampled or the hop limit is reached. 
% \else
%  An unbiased estimator for conn(c,d). To enable faster convergence, we build a k-hop reachability index~\cite{cheng2014efficient} on the KG instance space and only sample eligible neighbours that satisfy the hop constraint. Due to space limits, the detailed algorithm and theoretical analysis are presented in our technical report~\cite{ncexplorerfull}.
\fi


==> sections/revision_response.tex <==

\title{Revision Response}
\noindent{Dear Reviewers:}

We greatly appreciate your valuable feedback, which has helped us improve our paper. Following your suggestions, we have undertaken substantial revisions to refine our work. Major changes are marked \revision{\textbf{in blue}}. Below is a summary of the key changes made in this revision.

\section{summary of changes}
\begin{enumerate}
  \item In the introduction (Sec. \ref{chap:introduction}), we have added the main technical challenges of the roll-up and drill-down operations.
  \item In the related work (Sec. \ref{chap:related_work}), we have added the limitations of the existing approaches.
  \item In the framework description (Sec. \ref{chap:architecture}), we have added a system architecture diagram.
  \item We have re-arranged the subsections of the framework description (Sec. \ref{chap:architecture}) to align with the evaluations.
  \item In the evaluation (Sec. \ref{chap:evaluation}), we have added the overhead of building reachability index. 
  \item In the evaluation (Sec. \ref{chap:evaluation}), we have added a user study with roll-up and drill-down for a targeted use case.
  \item We have released a full report with additional content related to: algorithm of our sampling approach with the k-hop reachability index, detailed descriptions of our experiments, case studies and demo interfaces~\cite{ncexplorerfull}.
\end{enumerate}

\section{response to reviewer 1}
\review{1}The proposed work is somehow incremental with limited novelty. \\
\detailedComment{1}The paper fails to provide strong foundations for the proposed approach for capturing the hierarchical semantics. For example, developing a system like NCExplorer will face several technical problems. What are these technical problems? how does NCExplorer guarantee to solve them? The contribution would be more substantial if the authors clarified the system architecture of NCExplorer and the main challenges addressed by each component in the system. \\

\response
Thanks for your constructive feedback. 
Please kindly note that our proposed system does \emph{not} propose a semantic hierarchy. Instead, we rely on the ontology of the KG to enable the roll-up and drill-down analysis. We refer to the response of O2 for more discussions on this issue.

There are two main technical challenges for roll-up and drill-down operations, respectively. 

In roll-up operations, the key challenge is to identify relevant news articles that correspond to selected roll-up concepts. This task is complicated by the fact that roll-up concepts are part of the Knowledge Graph's (KG) ontology space, while the news articles' entities often belong to the KG's instance space. To address this, we develop a relevance measure linking these two spaces and devise efficient path-based methods to quickly pinpoint relevant articles for roll-up analysis.

For drill-down operations, the key challenge lies in the effective ranking of sub-topic concepts to facilitate in-depth drill-down investigations by analysts. This task is particularly demanding due to the vast array of potentially relevant concepts suitable for drill-down analysis. To meet this challenge, we have designed a ranking framework according to the business requirements, incorporating three critical dimensions: coverage, specificity, and diversity.


%To integrate the ontology space of KG with the hierarchical semantics of news documents, there are two main challenges. 
%First, the relevance between a KG instance (e.g. \kgentity{Ford Motor}) entities and a news article can be measured by existing keyword matching algorithms; however, to go beyond KG instance to KG concepts, we need a measurement that reflects the content of news articles. \kgentity{Ford Motor} can be rolled-up into concepts like \kgentity{American Company}, \kgentity{EV Company}. Each concept's relevance to an article varies according to the content. For a report on business impact of Russian-Ukraine conflict, \kgentity{American Company} is more relevant than \kgentity{EV Company}. We use the paths between a concept node (\kgentity{American Company}) to other link instance nodes in the news report (e.g. \kgentity{sanction}, \kgentity{export}) to proximate this relevance score. This score is expensive to compute due to the big size of KG. Sec. \ref{sec:ranking} defines the relevance score and Sec. \ref{sec:connectivity_score_estimation} describes our sampling technique to speedup the calculation.

%The second challenge is to rank the subtopics linked to query results (Sec. \ref{sec:subtopic}). For the task of risk management, the goal is to discover unknown emerging trend. Subtopics with high coverage scores alone is not meaningful to the analysts. We designed a score that  considers the diversity of instance entities linked to the concept as well as the specificity score of the concept.

In the revision, we have added the above discussion in the introduction (Sec. \ref{chap:introduction}). 

\review{2}The systematic aspects for capturing the hierarchical semantics are unclear. \\
\detailedComment{2}The paper would be more substantial if the authors provided a detailed algorithm for capturing the hierarchical semantics of documents and interlinking them to existing concepts and instances in the KG. The reader would be interested in understanding the system's ability to process and organize a continuous flow of news articles. LLM-based approach for ontology and context relevance is unclear. \\

\response
To capture the hierarchy, we use the \kgentity{broader} relationship in the KG ontology space to enable \rollup and \drilldown operations.
For example, in Fig \ref{fig:kg_toy_sample}, \kgentity{MIT Alumni} is associated with \kgentity{MIT People} via the edge type \kgentity{broader}. We have added this clarification in Section \ref{sec:ranking}.

\noindent\textbf{System Diagram.}
We have added a system architecture diagram (Fig.~\ref{fig:architecture}) for the framework description. The framework can process a continuous stream of news articles. Each document goes through a standard pipeline of natural language processors (NLP). We use the Spacy\cite{honnibal2017spacy} library for this task. This NLP pipeline transforms a text document into a list of KG instance entities. 
We then calculate the ontology and context relevance scores for each document based on the extracted entities.
We included the discussions in Section~\ref{chap:architecture}. 
%The edge concepts connected to these instance entities are used to calculate $cdr(c, d)$.

\noindent\textbf{LLM Component.}
We would like to highlight that the LLM is not used for explicitly capturing ontology and context relevance. Instead, LLM is only used to perform the final re-ranking of top-K results generated by \framework, due to time and cost feasibility in the business environment. 
%Table \ref{tab:gpt-ndcg-impact} shows LLM can boost NDCG@1 score by 6.75\% which means it can detect additional semantic information that KG network fail to capture. Due to the context length limitation and cost issue, it is not feasible to use LLM to calculate the relevance score for each $cdr(c, d)$. 
We have added this clarification in the evaluation (sec. \ref{sec:relevance-study}). \\

\review{3}
The evaluation did not analyze the cost of constructing the KG.\\
\detailedComment{3}The core contribution of NCExplorer is the construction of ontology and context relevance for news documents. The evaluation would be stronger if the authors analyzed the cost of the construction process and compared it against existing systems. The prompt-based approach is also not justified. For example, The reason for requesting a rating between 0 and 5 in the provided prompt is unclear. Do the GPT specifications specifically recommend this range? Alternatively, would using a rating out of 10 be more appropriate? The formalization of the prompts needs clarification to ensure consistency and understanding. \\


\response 
Please note the KG construction is orthogonal to the contributions of this work and our proposed system can potentially work with any KG. 

\noindent\textbf{Computational Costs of Ontology and Context Relevance.}
We have evaluated the overall index costs in Fig.~\ref{fig:document_indexing_time} of the revised paper. We also include the time break down in the above Figure of this page. 
The dominant component is entity linking which takes about 90\% of total processing time. 
%This overhead is incurred for all KG-based report and takes extra 2 seconds compared to non-KG based methods. 
The costs for ontology and context calculation only take less than 8\% of the total computing time. 
Please kindly note that optimizing entity linking efficiency is orthogonal to this work. We have added this experiment to the extended report\cite{ncexplorerfull}. 


\begin{figure}[t]
    
    \includegraphics[width=\linewidth]{images/output-figure1.pdf}
    \vspace{-1em}
    \label{fig:indexing-overhead-analysis}
\caption{Ontology relevance computing overhead analysis}
    \vspace{-1em}
\end{figure}

\noindent\textbf{GPT Evaluation.}
% We redesigned the prompt as shown below:\\
% \noindent\fbox{
%   \parbox{0.95\linewidth}{%
%     \textbf{original prompt}: $<$news article$>$. Is this article related to $<$topic$>$. please give a rating between 0.000 and 5.000, with 5.000 being most relevant. only give three decimal digits.
%     }
% }
% \noindent\fbox{
%   \parbox{0.95\linewidth}{%
%     \textbf{redesigned prompt}: Given the following news article: $<$news article$>$. Please assess its relevance to the topic:  $<$topic$>$.  Provide an integer rating between 0 and 10, with 10 indicating the highest relevance.
%     }
% }
We have re-run the experiment using 0-10 scale. An independent samples t-test against original 0-5 scale experiment shows a p-value of 0.878. Our chosen significance level (alpha) is 0.05. The p-value is bigger than alpha, rejecting the null hypothesis, demonstrating that different scales do not affect evaluation results. This finding is consistent with the effect of scales in relevance assessments for crowdsourced participants\footnote{\url{https://www.sciencedirect.com/science/article/abs/pii/S0306457321001734}}. We added this additional experiment in extended report\cite{ncexplorerfull}. \\

\section{response to reviewer 2}
\review{1} Challenges are not stated in introduction nor become clear later in the paper. Why using different kind of operations is hard to solve? Please add challenges to introduction.\\


\response
Thanks for the feedback. Please refer to the response for O1 of Reviewer 1 regarding the discussion. \\

\review{2} Problem statement is not defined. Please add it at the beginning of Section 3 and evaluate the effectiveness of the proposed approach with respect to these metrics in Section 4. \\

\response Thanks for the feedback. We have added the problem statement of \rollup operation at Definition \ref{def:rollup} and \drilldown operation at Definition \ref{def:drilldown}. The \rollup operation finds top-k most relevant documents. The \drilldown operation finds top-k most useful subtopics with the usefulness defined as $sbr(c, Q)$.


\review{3} Section 2 does not describe the limitations of the existing approaches. Please add.\\

\response Thanks for the feedback. Limitations have been added in Section \ref{chap:related_work}. The two main categories of existing approaches are embedding based semantic relevance algorithms and graph based algorithms. The main issue with embedding-based approaches is the lack of explicit explanation which is a requirement for due diligence where each claim need to be backed with clear evidence. For graph-based approaches, existing work largely focus on augmenting the robustness of search results by adding hidden KG instance nodes as query keywords. They do not integrate the KG concept space to provide an OLAP-like exploration experience.


\section{response to reviewer 3}

\review{1} Conduct a user study with drill-down and roll-up for the targetted use case (W1). W1: The paper did not evaluate the main use-case of the paper: drill-down and roll-up for risk analysis and due diligence. This should be evaluated in a user study: real analysts (e.g. finance/business students) use the operations and demonstrate that the technique improves performing due diligence by some metric (e.g. speed of performing analysis). \\

\response Thanks for your feedback. 
For this revision, we have worked with our compliance team to create a task list resembling a standard set of investigative inquiries. 
The participants are required to investigate issues like: \emph{Find out the \textbf{names of Switzerland Banks} with reports related to \textbf{money laundering}.}
Given the open-ended nature of these tasks, we have set a fixed duration of 2 minutes and use the number of distinct relevance cases found as a performance metric. This task design mirrors the requirement of Suspicious Activity Reports (SARs)\footnote{https://legal.thomsonreuters.com/en/insights/articles/what-is-a-suspicious-activity-report}, where financial institutions have to file findings within a limited time once a potential criminal activity is identified. 

% The list of questions are as follow: 
% \begin{enumerate}
%   \item Find out the \textbf{categories of commercial crime} involves \textbf{Credit Suisse}.
%   \item Find out the \textbf{categories of commercial crimes} involves \textbf{Banks of Switzerland}.
%   \item Find out the \textbf{names of Switzerland Banks} with reports related to \textbf{commercial crimes}.
%   \item Find out the \textbf{names of Switzerland Banks} with reports related to \textbf{money laundering}.
%   \item Find out the \textbf{categories of commercial crime} involves \textbf{FTX}. 
%   \item Find out the \textbf{categories of commercial crimes} involves \textbf{Bitcoin exchanges}.
%   \item Find out \textbf{the names of Bitcoin exchanges} with reports related to \textbf{commercial crimes}.
%   \item Find out the \textbf{names of Bitcoin exchanges} with reports related to \textbf{money laundering}. 
% \end{enumerate}

%We built two search interfaces with a common corpus. Keyword search with BM25\cite{robertson2009probabilistic} algorithm is used as a baseline.
We recruited 10 financial professionals for this study. 
Using \framework, professionals can generate more answers within the same time limit than the existing keyword match-based method adopted in the corporation, as shown in Table~\ref{tab:productivity-gain-study}. We also asked a subjective question \kgentity{How likely are you to recommend this tool to due diligence professionals?} and got an average rating of 8.1/10. 
We have added the key description and main results in Sec. \ref{sec:rollup-drilldown-study} of the revised paper and included a detailed description of the study in the extended report\cite{ncexplorerfull} due to space limit. 

%\begin{table}[ht]
%\centering
%\include{figures/productivity_gain_study}
%  \label{tab:productivity-gain-study}
%\end{table}

 




\review{2} Compare this to a GPT-only solution with generated prompts (W2). W2: While the paper uses GPT models to rank documents, can the models be used to construct a solution? For example, using the example in the paper, a prompt might look like "Summarize FTX's involved in fraud with links or snippets of the most relevant articles." One challenge could be the staleness of the GPT's model.\\ 

\response 
Thanks for the comments. %As suggested, we feed the query in relevance evaluation (Sec. \ref{sec:relevance-study}) into GPT-3.5-turbo with the prompt
%\noindent\fbox{
%  \parbox{0.95\linewidth}{%
%    Please find news reports related to $<$Insert Topics Here$>$ with reference link.
%}}
As suggested, we employed a GPT-only solution but the LLM failed to produce desirable answers due to the staleness of the model. %In many cases, we obtain the following responses:

%All queries fail to generate required reponses. Instead GPT provides suggestions similar to the response below:\\
% \noindent\fbox{
%   \parbox{0.95\linewidth}{%
    
%    I'm unable to provide real-time news reports or access the internet for reference links as my knowledge is based on information available up to January 2022. To find the latest news reports related to "Lawsuits," I recommend visiting reputable news websites or using a search engine. Here are some trusted news sources where you can search for lawsuit-related news:

% 1. Reuters: https://www.reuters.com/\\
% 2. Bloomberg: https://www.bloomberg.com/\\
% 3. CNBC: https://www.cnbc.com/\\
% 4. The Wall Street Journal: https://www.wsj.com/\\
% 5. BBC News: https://www.bbc.com/news\\
% 6. The New York Times: https://www.nytimes.com/\\
% 7. CNN: https://www.cnn.com/\\

% You can visit these websites and use their search functions to find the latest news reports and articles on lawsuits. Simply enter "Lawsuits" or specific lawsuit-related keywords in the search bar to access relevant news articles with reference links.
% }}

 One potential approach is to utilize the responses from \framework as prompts for GPT models. Nonetheless, this strategy involves considerable expenses for businesses. Despite this, integrating KG with GPT models presents a promising avenue. We discuss it as a future work.  \\

\review{3} Show the overhead of computing and maintaining the reachability index (D2). D2: The paper shows the benefit of random sampling and the reachability index technique for connectivity. However it does not show the upfront cost to compute or the overhead of maintaining the index as new documents are added to the corpus. \\


\response
 The DBPedia KG we used contains 5.2 million nodes and 27.9 million edges. The overhead of computing reachability index is 260 seconds with 100GB of memory usage. This index is updated every time a new version of KG is released. Current release frequency is roughly every 3 months\footnote{\url{https://www.dbpedia.org/resources/snapshot-release/}}. We added this result in Section~\ref{sec:connectivity_score_estimation}.
\\

\review{4} The paper is quite short, consider expanding on the topics raised in the reviews to help reader understanding.

\response
Thanks for this suggestion. We've written to the chair for permission to extend the page limit. Unfortunately, we are required to stick within 6 pages. We released a full report at\cite{ncexplorerfull} with additional algorithm, proof, evaluation and case studies. We also added pointer in current paper to the full report to help the reader explore deeper on certain topics. 
\\



\setcounter{section}{0}
\setcounter{figure}{0}    

